Space Decomposition for Sentence Embedding

Determining sentence pair similarity is crucial for various NLP tasks. A common technique to address this is typically evaluated on a continuous semantic textual similarity scale from 0 to 5. However, based on a linguistic observation in STS annotation guidelines, we found that the score in the range [4,5] indicates an upper-range sample, while the rest are lower-range samples. This necessitates a new approach to treating the upper-range and lower-range classes separately. In this paper, we introduce a novel embedding space decomposition method called MixSP utilizing a Mixture of Specialized Projectors, designed to distinguish and rank upper-range and lower-range samples accurately. The experimental results demonstrate that MixSP decreased the overlap representation between upper-range and lower-range classes significantly while outperforming competitors on STS and zero-shot benchmarks.

==> Overlap___________sct.tex <==

\subsection{\hl{Embedding Space Analysis}} \label{subsec:cosine}
%
% ใส่ข้อมูลตรงนี้เพิ่ม
In this section, we analyze the quality of the embedding produced by different methods using the alignment and uniformity metrics~\cite{gao-etal-2021-simcse}. 
%
Alignment measures the distance in the embedding space between positive sentence pairs ($x, x^{+}$) with STS scores of 4 to 5 ($p_{\text {pos}}$):
%
\vspace{-2mm}
\begin{equation} 
% \resizebox{1\hsize}{!}
\begin{aligned}
\ell_{\text {align }} \triangleq \mathbb{E}_{\left(x, x^{+}\right) \sim p_{\text {pos }}}\left\|f(x)-f\left(x^{+}\right)\right\|^2
\end{aligned}
\vspace{-2mm}
\label{eq:alignment}
\end{equation}
%
On the other hand, uniformity measures how dispersed the sentence pairs are in the embedding space:
%
\vspace{-2mm}
\begin{equation} 
% \resizebox{1\hsize}{!}
\begin{aligned}
\ell_{\text {uniform }} \triangleq \log \quad \underset{\substack{x, y \stackrel{i . i . d .}{\sim} p_{\text {data }}}}{\mathbb{E}} e^{-2\|f(x)-f(y)\|^2}
\end{aligned}
\vspace{-2mm}
\label{eq:uniform}
\end{equation}
%
Thus, the two metrics try to find a balance between correctness and sparsity.


\begin{table}[h]
% \vspace{-1mm}
\hspace*{-4mm}
\renewcommand{\arraystretch}{\setwidth}
\centering
\setlength\doublerulesep{3pt}
\scalebox{0.7}{
\setlength{\tabcolsep}{2pt}
%\fontsize{10pt}{12pt}\selectfont
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} &
  \multicolumn{3}{c|}{\smallmodel{\textbf{BERT-Tiny}}} &
  \multicolumn{3}{c|}{\mediummodel{\textbf{BERT-Small}}} &
  \multicolumn{3}{c}{\largemodel{\textbf{BERT-Base}}} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Align}}} &
  \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Uniform}}} &
  \rotatebox[origin=c]{90}{\textbf{STS}} &
  \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Align}}} &
  \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Uniform}}} &
  \rotatebox[origin=c]{90}{\textbf{STS}} &
  \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Align}}} &
  \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{\textbf{Uniform}}} &
  \rotatebox[origin=c]{90}{\textbf{STS}} \\ \hline
SimCSE &
  \multicolumn{1}{c|}{0.159} &
  \multicolumn{1}{c|}{-2.081} &
  61.77 &
  \multicolumn{1}{c|}{0.185} &
  \multicolumn{1}{c|}{-2.203} &
  69.04 &
  \multicolumn{1}{c|}{0.243} &
  \multicolumn{1}{c|}{\textbf{-2.725}} &
  76.85 \\ \hline
DCLR &
  \multicolumn{1}{c|}{0.142} &
  \multicolumn{1}{c|}{-1.790} &
  47.31 &
  \multicolumn{1}{c|}{0.217} &
  \multicolumn{1}{c|}{\textbf{-2.273}} &
  61.67 &
  \multicolumn{1}{c|}{0.270} &
  \multicolumn{1}{c|}{-2.498} &
  78.31 \\ \hline
DiffCSE &
  \multicolumn{1}{c|}{\textbf{0.123}} &
  \multicolumn{1}{c|}{-1.618} &
  61.78 &
  \multicolumn{1}{c|}{0.194} &
  \multicolumn{1}{c|}{-2.093} &
  67.86 &
  \multicolumn{1}{c|}{\textbf{0.119}} &
  \multicolumn{1}{c|}{-1.459} &
  \textbf{80.59} \\ \hline
SCT &
  \multicolumn{1}{c|}{0.248} &
  \multicolumn{1}{c|}{\textbf{-2.439}} &
  \textbf{71.79} &
  \multicolumn{1}{c|}{\textbf{0.124}} &
  \multicolumn{1}{c|}{-1.417} &
  \textbf{75.33} &
  \multicolumn{1}{c|}{0.191} &
  \multicolumn{1}{c|}{-2.218} &
  76.91 \\ \hline
\end{tabular}
}
\vspace{-2mm}
\caption{\label{font-table} The alignment (align), uniformity (uniform), and STS-B scores on BERT-Tiny, BERT-Small, and BERT-Base.}
\vspace{-4mm}
\label{tab:align_uniform_table}
\end{table}


\begin{figure}[h]
\hspace*{-3.5mm}
\centering
\newcommand{\figwidth}{5.0cm}
\begin{subfigure}{\figwidth}
\vspace{-1mm}
\includegraphics[width=\textwidth]{images/all_PLMs_Alignment score.pdf}
\vspace{-7mm}
\caption{Alignment score}
\label{fig:alignment.all}
\end{subfigure}
%
\begin{subfigure}{\figwidth}
\vspace{-1mm}
\includegraphics[width=\textwidth]{images/all_PLMs_Uniformity score.pdf}
\vspace{-7mm}
\caption{Uniformity score}
\label{fig:uniformity.all}
\end{subfigure}
%
\begin{subfigure}{\figwidth}
\vspace{-1mm}
\includegraphics[width=\textwidth]{images/all_PLMs_Overlapped area.pdf}
\vspace{-7mm}
\caption{Overlapped area}
\label{fig:overlap.area.all}
\end{subfigure}
\vspace{-2mm}
\caption{The scatter plot of alignment, uniformity, and overlapped area (Y-axis) compared to the average Spearman's rank correlation (X-axis)(Table~\ref{tab:sts_tasks}) on BERT-Tiny, -Small, and -Base. We also evaluate the Pearson correlation coefficient (numbers shown are absolute values) of the X and Y axis.}
\vspace{-4mm}
\label{fig:scatter.all.all}
\end{figure}

\begin{figure*}[htpb]
\hspace*{-3.5mm}
\centering
\newcommand{\figwidth}{5.0cm}
\begin{subfigure}{\figwidth}
\includegraphics[width=\textwidth]{images/ridgeplot.model_type-BERT-Tiny.sts-stsb_test-set.changed-linestyle.pdf}
\caption{BERT-Tiny}
\label{fig:sim-dist.stsb.bert-tiny}
\end{subfigure}
%
\begin{subfigure}{\figwidth}
\includegraphics[width=\textwidth]{images/ridgeplot.model_type-BERT-Small.sts-stsb_test-set.changed-linestyle.pdf}
\caption{BERT-Small}
\label{fig:sim-dist.stsb.bert-small}
\end{subfigure}
%
\begin{subfigure}{\figwidth}
\includegraphics[width=\textwidth]{images/ridgeplot.model_type-BERT-Base.sts-stsb_test-set.changed-linestyle.pdf}
\caption{BERT-Base}
\label{fig:sim-dist.stsb.bert-base}
\end{subfigure}
\vspace{-2mm}
\caption{Cosine similarity distributions for BERT-Tiny, BERT-Small, and BERT-Base.}
\vspace{-5mm}
\label{fig:sim-dist.stsb.all}
\end{figure*}



%
Due to the trade-off nature of these two measures, no method dominates others in alignment and uniformity simultaneously. 
%
The exact nature of the trade-off between these metrics is unclear, and its relationship to STS performance is not apparent.
%
We also confirm this finding in Figures~\ref{fig:alignment.all} and \ref{fig:uniformity.all}.
%
We calculate the Pearson correlation coefficient on STS and alignment/uniformity scores in Table~\ref{tab:align_uniform_table}.
%
The scatter plot highlights that there are only weak relationships between these measures and STS scores.






Let us now consider cosine similarity distributions for the STS score ranges of  [0,3] (the rank score of irrelevance sentence pairs) and  (3,5] (the rank score of relevance sentence pairs) using the STS-B benchmark dataset.
%
Figures~\ref{fig:sim-dist.stsb.bert-tiny}, \ref{fig:sim-dist.stsb.bert-small}, and~\ref{fig:sim-dist.stsb.bert-base} shows distribution plots for BERT-Tiny, BERT-Small, and BERT-Base, respectively.
%
We derive a confusion-matrix-like measure to provide more insight into the behavior of our embedding space.
%
In particular, we compute the overlapped density area by estimating the densities using the Gaussian kernel density estimate.
%
This measure indicates the chance that sentence pairs from the two ranges can be confused with each other.  

The overlapped areas of each plot are displayed in Table~\ref{tab:over_lap_area}.
%
Since the two STS score ranges are mutually exclusive, we want the overlapped areas to be as close to zero as possible.
%
As can be seen, SCT has the smallest overlap in the case of BERT-Tiny and BERT-Small, while DiffCSE is the best performer for BERT-Base.
%
These results conform with the STS scores shown in Table~\ref{tab:sts_tasks} that SCT tends to perform better than other methods when the model has less than 100M parameters. 
%
Moreover, the overlapped area has a high correlation with STS rank correlation score as shown in Figure~\ref{fig:overlap.area.all}. 
%
It has a Pearson correlation of 56.87 which is much larger than the number from alignment and uniformity metrics.
%
We recommend this measurement instead of alignment or uniformity to analyze the goodness of embedding space.
%
\begin{table}[H]
% \vspace{-3mm}
\hspace*{-4mm}
\renewcommand{\arraystretch}{\setwidth}
\centering
\setlength\doublerulesep{3pt}
\scalebox{0.8}{
\setlength{\tabcolsep}{2pt}
%\fontsize{10pt}{12pt}\selectfont
\begin{tabular}{l|c|c|c|c}
\hline
\multicolumn{1}{c|}{\textbf{Models}}  & \textbf{SimCSE} & \textbf{DCLR} & \textbf{DiffCSE} & \textbf{SCT} \\ \hline
\smallmodel BERT-Tiny  & 0.610	& 0.579	& 0.582	& \textbf{0.477} \\ \hline
\mediummodel BERT-Small & 0.495	& 0.517	& 0.525	& \textbf{0.469} \\ \hline
\largemodel BERT-Base  & 0.475 & 0.514 & \textbf{0.426} & 0.438 \\ \hline
\end{tabular}
}
\vspace{-2mm}
\caption{\label{font-table} The overlapped area of similarity distribution plots on STS-B test set as shown in Figure ~\ref{fig:sim-dist.stsb.all}.}
\vspace{-4mm}
\label{tab:over_lap_area}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Spearman correlation for each group (1-3,3-5) %%%%
%% [[TODO]] 


